Multi-View Learning for Vision-and-Language Navigation

Learning to navigate in a visual environment following natural language instructions is a challenging task because natural language instructions are highly variable, ambiguous, and under-specified. In this paper, we present a novel training paradigm, Learn from EveryOne (LEO), which leverages multiple instructions (as different views) for the same trajectory to resolve language ambiguity and improve generalization. By sharing parameters across instructions, our approach learns more effectively from limited training data and generalizes better in unseen environments. On the recent Room-to-Room (R2R) benchmark dataset, LEO achieves 16% improvement (absolute) over a greedy agent as the base agent (25.3% $\rightarrow$ 41.4%) in Success Rate weighted by Path Length (SPL). Further, LEO is complementary to most existing models for vision-and-language navigation, allowing for easy integration with the existing techniques, leading to LEO+, which creates the new state of the art, pushing the R2R benchmark to 62% (9% absolute improvement).

==> 09_ack.tex <==
\section*{Acknowledgments}
%We thank the anonymous reviewers for their insightful comments, NSF IIS-1703166, DARPA's CwC program through ARO W911NF-15-1-0543, and the Allen Institute for Artificial Intelligence. Qiaolin Xia was funded by the China Scholarship Council (grant no. 201806010268).
